Cloud Service Matchmaking Approaches: A Systematic Literature Survey

Service matching concerns finding suitable services according to the service requester's requirements, which is a complex task due to the increasing number and diversity of cloud services available. Service matching is discussed in web services composition and user oriented service marketplaces contexts. The suggested approaches have different problem definitions and have to be examined closer in order to identify comparable results and to find out which approaches have built on the former ones. One of the most important use cases is service requesters with limited technical knowledge who need to compare services based on their QoS requirements in cloud service marketplaces. Our survey examines the service matching approaches in order to find out the relation between their context and their objectives. Moreover, it evaluates their applicability for the cloud service marketplaces context.

==> overview.tex <==
\section{An Overview of Existing Approaches} 
This section categorises the proposed solutions to service matching problem as: syntactic, ontology based and Fuzzy Set Theory based. Some 
approaches combine several techniques. This categorisation is based on the statements of the authors of the respective papers. The aim of this 
categorisation is to follow the discourse in literature and identify connections between the proposed solutions, i.e. issues in existing 
approaches identified by others and how the newer approaches build up on former related work.
%\hl{there are two papers making this kind of categorisation: \cite{yu2008non}\cite{tuw2011qos} chapter 1.4.2} 

\subsection{Syntactic approaches}\label{sec:syntacticApp} 
Syntactic approaches, for example proposed by \cite{eleyan2011service}, \cite{kritikos2009mixed} and \cite{yu2007efficient}, take the 
service request as a set of constraints and the result set as a subset of all service descriptions which satisfy these constraints, i.e. a 
constraint satisfaction problem (CSP). They utilise mathematical models to describe the problem and then apply techniques such as Constraint 
Programming \cite{rossi2006handbook}, Mixed Integer Programming \cite{leyffer2012mixed}, and Analytic Hierarchy Process \cite{saaty1990make}. 
Other points common among these approaches are the ranking and the relaxation steps. To enhance the results after the initial matchmaking, they 
are ordered according to the service requester's priorities (ranking) \cite {eleyan2011service}, and non-exact matches which satisfy the most 
important constraints are added to them (relaxation) \cite{mobedpour2013user}. 

The matchmaking approach proposed by \cite{ruiz2005improving} is an early example of the application of CSPs to the service matching problem. 
\cite {kritikos2008evaluation} evaluates the algorithm proposed in \cite{ruiz2005improving} and two versions of the algorithm for unary 
constraints proposed in \cite{kritikos2007semantic} by their time performance and precision. The algorithm defined by \cite
{ruiz2005improving} in  \cite {ruiz2005improving} categorises the results only in exact matching and fail groups and places the service 
descriptions which are better than the request in the fail group. For these reasons, it exhibits lower precision than the other algorithms 
evaluated in \cite{kritikos2008evaluation}. The first algorithm proposed in \cite{kritikos2007semantic} addresses this problem and the second one 
proposes further categorisation of results in super, exact, partial and fail sets. The time performance experiments show that the first two 
algorithms are faster than the third algorithm, however they do not return partial matches which might help the service requester find an 
acceptable service description. 
%None of these three algorithms rank the results.

\cite{kritikos2009mixed} evaluates MIP versions of the \cite{ruiz2005improving}, two versions of A and a simpler version of B in \cite 
{kritikos2007semantic}. \cite{mobedpour2013user} builds on an MIP algorithm presented in \cite{kritikos2009mixed} and integrates it in a 
user-centered service selection system. 

It can be observed that the above presented related work focuses on time performance and on precision of the algorithms which take QoS 
requirements as numerical values. An exception to this observation is the system developed by \cite{mobedpour2013user} which shifts the focus 
to usability issues. Figure \ref{fig:matchersTaxC} shows the relations between constraint based approaches.
%\paragraph*{}\cite{yu2007efficient}, \cite{sarang2012clustering}, \cite{eleyan2011service} \hl{TODO describe further, see the experiment results}

\begin{figure}
  \centering
 \includegraphics[width=15cm,height=12cm]{graph.pdf}
  \caption{Constraint Programming Based Service Matchers in Literature}\label{fig:matchersTaxC}
\end{figure}
\subsection{Ontology Based Approaches}  

Ontology based approaches, such as the ones presented by \cite{d2008semantic}, \cite {liu2009weighted} and \cite {liu2011syntactic}, 
utilise OWL-S to capture comprehensive descriptions of cloud services and utilise ontology reasoners to match services to service queries. These 
systems provide accurate results with the help of detailed comparison of semantic data, however they give up efficiency for accuracy\cite 
{tuw2011qos}. The source of the problem is the performance problems of ontology reasoners. 

%use source \cite{dong2012Semantic} %here goes summary of Semantic Web Service matchmakers: state of the art and challenges   

%\hl{You can also cite like Kiritikos et al. [4] presented a study or 
%found that it is like this. The approach introduced by Kritikos et al.[4] does ... Kritikios et al.[4] conclude/compare/define... }   

\subsection{Fuzzy Set Theory Based Approaches} \label{subsec:fuzzyApp}
Approaches presented by \cite{wang2009qos}, \cite{mobedpour2013user} and \cite{bacciu2010adaptive} utilise fuzzy set theory to 
categorize and match services to the service requester's query. The approaches by \cite{wang2009qos} and \cite {mobedpour2013user}  utilise 
various techniques to map linguistic terms such as moderate, good, very good to actual values in service descriptions. They achieve this by:
\begin{itemize}
\item building up intuitionistic fuzzy sets using consumers perception 
\item clustering
\end{itemize} 

On the other hand, the method proposed by \cite{bacciu2010adaptive} does not apply linguistic term matching, but uses fuzzy membership values 
for providing variational scope.

\cite{wang2009qos} aggregates the perceived quality expressed in linguistic terms to form an objective service description and weights for QoS properties. 
The disadvantage of this approach \cite{wang2009qos} is its demand on a great amount of user input. It expects the users to look at each service for each QoS property 
and tell the system their opinion. This is not feasible to be used as a standalone in the TRESOR/TCC context. For the attributes which cannot 
be measured, it provides a systematical way to combine former user reviews with the service requester's priorities.

\cite{mobedpour2013user} uses a symbolic clustering algorithm (SCLUST) with the assumption that fuzzy values are 
only meaningful for numeric QoS properties. SCLUST places service descriptions on one of the intervals corresponding to good, medium, poor. The values for the
limits of the intervals are calculated relatively considering all the services in the repository.

\cite{bacciu2010adaptive} focuses on QoS requirements which state soft constraints and utilises trapezoidal fuzzy numbers to address this issue i.e.
a QoS requirement of availability between 95\% and 99\% is mapped to acceptable answers ranging between 94\% and 100\% where the acceptability degree to values
graph forms a trapezoid.
 
%\hl{Can the enumeration type QoS properties be handled with fuzzy set intersection operator?} 

\subsection{Hybrid Approaches } 
\paragraph*{Fuzzy and Syntactic Approaches} In the user-centered prototype presented by \cite{mobedpour2013user}, constraint based and fuzzy 
approaches are combined. For constraint based, they use an algorithm presented in \cite{kritikos2009mixed}. See Subsection \ref{subsec:fuzzyApp} 
for the description of the fuzzy component. 

\paragraph*{Fuzzy and Semantic Approaches} The fuzzy matching for numerical values described in \cite{bacciu2010adaptive}, is part of the Dino 
Broker\cite{mukhija2007qos} implemented as part of the EU funded Sensoria Project. Dino Broker aims to achieve "dynamic discovery and invocation in open dynamic environments". In this context, service selection or matching is 
just one of the components in the system. The authors define the stages of service composition as service discovery, selection, binding, delivery, 
monitoring and adaptation. The open dynamic environment means that services might have changing properties in run-time (dynamic) and they might be 
entering to, and exiting from, the environment (open). Dino Broker uses OWL-S descriptions of services to perform functional properties and API matching.
%\cite{liu2012fuzzy}  also in this category, maybe write later on it.
\paragraph*{Syntactic and Semantic Approaches} 
%Input alignment is realized with the help of semantic technologies and the actual matchmaking is done with constraint programming. 
The publications from the S-Cube project \cite{scube} are complementary \cite {kritikos2006semantic}, \cite{kritikos2007semanticover}, \cite
{kritikos2007semantic}, \cite{kritikos2008evaluation}, \cite{kritikos2009mixed},\cite{kritikos2012optimal}. Their main idea is that the semantic 
approaches which use ontology reasoners have performance problems, while the constraint based approaches deliver inaccurate results. They conclude 
that the solution should utilize the best of both worlds.
%~ mathias :2.1.4.3: "The main reason of inaccuracy in constraint based approach is the metric incompatibility among service descriptions and service requests." -
% Warum macht man so einen riesen Aufwand für Input Matching, wenn man auch einfach die Eingabewerte begrenzen kann?
These publications claim that the main reason of inaccuracy in constraint based approach is the metric incompatibility among service descriptions 
and service requests. The solution proposed in the S-Cube project defines QoS metrics in QoS requests and service specifications in OWL-Q \cite 
{kritikos2006semantic}, \cite {kritikos2007semanticover} and aligns the units of metrics of all available service descriptions in the repository. 
After the alignment of metrics, the constraint programming algorithms proposed in \cite{ruiz2005improving}, \cite{kritikos2007semantic} and  \cite 
{kritikos2009mixed} are applied and evaluated in their time performance and accuracy. See also Section \ref{sec:syntacticApp}. 

%\hl{verify \cite{jie2011dynamic}, \cite{palmonari2009effective} } 

\subsection{Fuzziness Considerations in Existing Approaches} \label{subsec:sourceofFuzzy}
The objective of the service matching process is to find the most suitable service for the service request. To provide detailed results, a service 
matcher should be able to evaluate to which extent a service matches the request. Namely, the service matcher should provide the service requester 
with details other than a definitive yes or no response. For this reason, some service matchers utilise sources of fuzziness. Three sources of 
fuzziness in existing service matching approaches are identified by Platenius et. al \cite {platenius2013survey}: 
\begin{itemize}
\item incomplete knowledge
\item variational scope
\item heuristics \& simplifications
\end{itemize}

Incomplete knowledge refers to how the matching approach deals with missing values for the input parameters, and can be considered in two ways:
\begin{itemize}
\item The service requester is not sure about all the constraints and therefore does not define a requirement for each property of the service
\item The service provider might not supply information for all the properties of the service. 
\end{itemize}

Variational scope can be introduced to a service matching approach in three ways: 
\begin{enumerate}
\item The matching of service description parameters to requirements 
with a certain amount of tolerance---assuming most requesters would accept a service with a value slightly different than the specified value
\item The parameters are specified with fuzzy terms such as "good" or "very fast"
\item The requirements are specified with their level of importance to the 
requester with qualifiers such as mandatory and optional. 
\end{enumerate}

A concrete example for the first type is the relaxation step which is suggested in \cite {mobedpour2013user}. An example for the second type can 
be found in \cite{wang2009qos} in the ranking of services based on weights assigned to QoS requirements by users.  

Heuristics are used to simplify the problem when the underlying mathematical modelling of the problem is 
NP-Hard or NP-Complete. However, the effects of these simplifications on the result set remains unclear.  

